Assessing the Frontier: Active Learning, Model Accuracy, and Multi-objective Materials Discovery and Optimization

Discovering novel materials can be greatly accelerated by iterative machine learning-informed proposal of candidates---active learning. However, standard \emph{global-scope error} metrics for model quality are not predictive of discovery performance, and can be misleading. We introduce the notion of \emph{Pareto shell-scope error} to help judge the suitability of a model for proposing material candidates. Further, through synthetic cases and a thermoelectric dataset, we probe the relation between acquisition function fidelity and active learning performance. Results suggest novel diagnostic tools, as well as new insights for acquisition function design.

==> te-distance.tex <==

\begin{tabular}{r|r|r|r}
\hline
$\rho\, (\text{Ohm}\cdot\text{cm})$ & $\kappa\, (W/mK)$ & Rank: $[\rho] = \text{Ohm}\cdot\text{cm}$ & Rank: $[\rho] = \text{Ohm}\cdot \text{m}$\\
\hline
130.00 & 0.38 & 1 & 185\\
\hline
0.26 & 48.70 & 2 & 1\\
\hline
0.01 & 44.49 & 3 & 2\\
\hline
0.00 & 44.49 & 4 & 3\\
\hline
0.00 & 40.29 & 5 & 4\\
\hline
0.00 & 34.50 & 6 & 5\\
\hline
\end{tabular}
